Learning Based Industrial Bin-picking Trained with Approximate Physics Simulator

In this research, we tackle the problem of picking an object from randomly stacked pile. Since complex physical phenomena of contact among objects and fingers makes it difficult to perform the bin-picking with high success rate, we consider introducing a learning based approach. For the purpose of collecting enough number of training data within a reasonable period of time, we introduce a physics simulator where approximation is used for collision checking. In this paper, we first formulate the learning based robotic bin-picking by using CNN (Convolutional Neural Network). We also obtain the optimum grasping posture of parallel jaw gripper by using CNN. Finally, we show that the effect of approximation introduced in collision checking is relaxed if we use exact 3D model to generate the depth image of the pile as an input to CNN.

==> bib2.tex <==
\small
\begin{thebibliography}{10}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{turkey} % Segmentation(rock crushing particle)
M. J. Turkey, 
``Automated Online Measurement of Limestone Particle Size Distributions using 
3D Range Data", 
J. of Process Control, vol. 21, pp. 254-262, 2011. 

\bibitem{Kristensen} % segmentation and pose detection of box shaped object
S. Kristensen et al., 
``Bin-picking with a Solid State Range Camera", 
Robotics and Autonomous Systems, vol. 35, pp. 143-151, 2001. 

\bibitem{Ghita} %range sensor, identify and grasp top most
O. Ghita and P. F. Whelan, 
``A bin picking system based on depth from defocus", 
J. Machine Vision and Applications, vol. 13, no. 4, pp. 234-244,
2003.

\bibitem{Kirkgaard} % segmentation and model maching by using HSC feature
J. Kirkegaard and T. B. Moeslund, 
``Bin-Picking based on Harmonic Shape Contexts and Graph-Based Matching", 
{\it Int. Conf. on Pattern Recognition}, vol. 2, pp. 581-584, 2006.

\bibitem{Fuchs} %ICP detection
S. Fuchs et al., 
``Cooperative Bin-Picking with Time-of-Flight Camera and Impedance Controlled DLR Lightweight Robot III", 
{\it IEEE Int. Conf. on Intelligent Robots and Systems}, pp.4862-4867, 2010.

\bibitem{Zuo} %coarse to fine: Stereo feature matching
A. Zuo et al., 
``A Hybrid Stereo Feature Matching Algorithm for Stereo Vision-Based Bin Picking", 
J. Pattern Recognition and Artificial Intelligence, vol. 18, no. 8, pp. 1407-1422. 2004.

\bibitem{Domae2014}
Y. Domae et al., 
``Fast Graspability Evaluation on Single Depth Maps for Bin Picking with General Grippers", 
{\it IEEE Int. Conf. on Robotics and Automation}, pp. 1197-2004, 2014.

\bibitem{Dupuis_08} %multiple candidate point bin-picking
D.C. Dupuis et al., 
``Two-Fingered Grasp Planning for Randomized Bin-Picking", 
{\it Robotics, Science and Systems 2008 Manipulation Workshop}, 2008.

\bibitem{icra13}
K. Harada et al., 
``Probabilistic Approach for Object Bin Picking Approximated by Cylinders", 
{\it IEEE Int. Conf. on Robotics and Automation}, pp. 3727-3732, 2013.

\bibitem{SII}
K. Harada et al., 
``Project on Development of a Robot System for Random Picking--Grasp/Manipulation Planner for a Dual-arm Manipulator--", 
{\it IEEE/SICE Int. Symposium on System Integration}, pp. 583-589, 2014.

\bibitem{Levine}
S. Levine et al., 
``Learning Hand-Eye Coordination for Robotic Grasping with Deep Learning and Large-Scale Data Collection", 
{\it Int. Symposium on Experimental Robotics}, 2016. 

\bibitem{case2016}
K. Harada et al., 
``Initial Experiments on Learning-Based Randomized Bin-Picking Allowing Finger Contact with Neighboring Objects", 
{\it IEEE Int. Conf. on Automation Science and Engineering}, pp. 1196-1202, 2016. 

\bibitem{Zeng}
A. Zeng et al., ``Robotic Pick-and-place of Novel Objects in Clutter with Multi-affordance Grasping and Cross Domain Image Matching", 
https://arxiv.org/abs/1710.01330

\bibitem{RefineNet}
G. Lin et al., ``RefineNet: Multi-Path Refinement Networks for High-Resolution Semantic Segmentation", 
https://arxiv.org/abs/1611.06612

\bibitem{Dexnet2}
J. Mahler et al., ``Dex-Net 2.0: Deep Learning to Plan Robust Grasps with Synthetic Point Clouds and Analytic Grasp Metrics", 
https://arxiv.org/abs/1703.09312

\bibitem{graspgan}
K. Bousmalis et al., 
`Using Simulation and Domain Adaptation to Improve Efficiency of Deep Robotic Grasping", 
https://arxiv.org/abs/1709.07857, 2017. 

%\bibitem{Dogar_RSS12}
%M. Dogar, K. Hsiao, M. Ciocarlie, and S. Srinivasa, 
%``Physics-based grasp planning through clutter", 
%Proc. of Robotics: Science and Ssystems, 2012.

\bibitem{Random}
L. Breiman, 
``Random Forests", 
Machine Learning, vol. 45, no. 1, pp. 5-32, 2001. 

\bibitem{Curtis}
N. Curtis and J. Xiao, 
"Efficient and Effective Grasping of Novel Objects through Learning and Adapting a Knowledge Base", 
{\it IEEE Int. Conf. on Intelligent Robots and Systems}, pp.2252-2257, 2008.

\bibitem{Lenz}
I. Lenz, H. Lee, and A. Saxena, 
``Deep Learning for Detecting Robotic Grasps", 
Int. J. Robotics Resaerch, vol. 34, no. 4-5, pp. 705-724, 2015. 

\bibitem{Pas}
A.t. Pas and R. Platt, 
``Using Geometry to Detect Grasps in 3D Point Clouds", 
Int. Symposium on Robotics Research, 2015. 

\bibitem{Ekvall}
S. Ekvall and D. Kragic, 
``Learning and evaluation of the approach vector for automatic grasp generation and planning", 
{\it IEEE Int. Conf. on Robotics and Automation}, 2007.

\bibitem{Harada_icra08}
K. Harada, K. Kaneko, and F. Kanehiro, 
``Fast Grasp Planning for Hand/Arm Systems Based on Convex Model", 
{\it IEEE Int. Conf. on Robotics and Automation}, pp. 1162-1168, 2008. 

\bibitem{icra14}
K. Harada et al., 
"Stabiltiy of Soft-Finger Grasp under Gravity", 
{\it IEEE Int. Conf. on Robotics and Automation}, pp. 883-888, 2014.

bibitem{Thrun}
S. Thrun et al., 
Probabilistic Robotics, MIT Press, 2005. 

\bibitem{Nagata10}
K. Nagata et al., 
``Picking up and Indicated Object in a Complex Environment", 
{\it Proc. of IEEE/RSJ Int. Conf. on Intelligent Robots and Systems}, 2010. 

\bibitem{CVFH}
A. Aldoma et al., 
``OUR-CVFH - Oriented, Unique and Repeatable Clustered Viewpoint Feature Histogram for 
Object Recognition and 6DOF Pose Estimation", 
Pattern Recognition, Springer, pp. 113-122, 2012. 

\bibitem{lccp}
C. M. Stein et al., 
``Object Partitioning using Local Convexity", 
{\it IEEE Int. Conf. on Computer Vision and Pattern Recognition}, 2014. 

\bibitem{pcl}
PCL-Point Cloud Library, 
http://pointclouds.org/

\bibitem{convex}
K. Mamou and G. Faouzi, ``A Simple and Efficient Approach for 3D Mesh Approximate Convex Decomposition", 
{\it IEEE Int. Conf. on Image Processing}, pp. 3501-3004, 2009. 

\bibitem{Relu}
Y. LeCun, Y. Bengio, G. Hinton, 
``Deep Learning", 
Nature, vol. 521, pp. 436-444, 2015. 

\bibitem{russakovsky2015imagenet}
O. Russakovsky et al., 
``Imagenet large scale visual recognition challenge", 
Int. J. of Computer Vision, 
vol. 115, no. 3, pp. 211-252, 2015. 

\bibitem{grauman2011visual}
K. Grauman and B. Leibe, 
Visual object recognition,
Synthesis lectures on artificial intelligence and machine learning, 
vol. 5, no. 2, pp. 1-181, 2011. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{thebibliography}
\normalsize

